Robust Implicit Backpropagation

Arguably the biggest challenge in applying neural networks is tuning the hyperparameters, in particular the learning rate. The sensitivity to the learning rate is due to the reliance on backpropagation to train the network. In this paper we present the first application of Implicit Stochastic Gradient Descent (ISGD) to train neural networks, a method known in convex optimization to be unconditionally stable and robust to the learning rate. Our key contribution is a novel layer-wise approximation of ISGD which makes its updates tractable for neural networks. Experiments show that our method is more robust to high learning rates and generally outperforms standard backpropagation on a variety of tasks.

==> scrap.tex <==
Use the same architecture and hyperparameters as given in the papers. We used three well established resources to guide our choice of hyperparameters \cite{pascanu2013difficulty}, \cite{klambauer2017self} and \cite{Goodfellow-et-al-2016}. All preprocessing was the same as in the paper or the data was pre-processed (e.g. already split into training and test sets). The loss functions are those used in the original papers.
%--------------------------------------------------
\paragraph{Hyperparameters}
\begin{itemize}
\item No momentum
\item No ridge regularization
\item Standard SGD (didn't use Adam)
\item Random seeds 1,2,3,...
\item Minibatch size 100.
\item Constant learning rate
\item Weight and bias initialization
\item Clipping
\end{itemize}






\begin{table}
\centering
\caption{Hyperparameter combinations}
\label{tb:hyperparameter_combinations}

\begin{tabular}{p{0.2\textwidth}p{0.3\textwidth}p{0.5\textwidth}}
\toprule
\textbf{Hyperparameter} & \textbf{Considered values} & \textbf{Reason}\tabularnewline
\midrule
Clipping threshold & $\{10,\infty\}$ & \cite{pascanu2013difficulty} use thresholds of $6, 8, 45$ and claimed that the performance is not sensitive to the threshold. The value of 10 is in the middle of these numbers and is thus a reasonable choice. \tabularnewline
\hline
Momentum & $\{0,0.9\}$ & 0.9 is a common value according to \cite[p. 294]{Goodfellow-et-al-2016} (and 0 corresponds to no momentum)\tabularnewline
\hline
Learning rate & $10^{\{1,0.5,0,-0.5,-1,-1.5,-2,-2.5,-3\}}$ & \cite{pascanu2013difficulty} and \cite{klambauer2017self} use learning rates in $10^{-\{0,1,2,3\}}$. Since we are interested in the robustness to the learning rate, we increased its granularity and maximum value. \tabularnewline
\hline
Ridge regularization & $\{0,10^{-4}\}$ & \cite{klambauer2017self} has regularization constants in $\in 10^{-\{3, 4, 5\}}$. We take the middle value (and 0 corresponds to no regularization). \tabularnewline
\hline
SGD type & \{ESGD, ISGD\} & - \tabularnewline
\hline
Random seed & \{1,2,...\} & - \tabularnewline
\bottomrule
\end{tabular}
\end{table}





\begin{table}
\centering
\caption{Hyperparameter fixed values}
\label{tb:hyperparameters_fixed}
\begin{tabular}{p{0.2\textwidth}p{0.3\textwidth}p{0.5\textwidth}}
\toprule
\textbf{Hyperparameter} & \textbf{Value} & \textbf{Reason}\tabularnewline
\midrule
Activation function & Arctan if sigmoid, Relu if non-sigmoid & Arctan and Relu are compatible with both ESGD and ISGD \tabularnewline
\hline
%Random seed & 1 & Each configuration is only run once\tabularnewline
%\hline
%Number epochs & 100 & Same as used in \cite{klambauer2017self} \tabularnewline
%\hline
Weight matrix initialization & $unif\left(-\sqrt{\frac{6}{n+m}},\sqrt{\frac{6}{n+m}}\right)$ (where $n$ = input size, $m$ = output size to layer) & Follows advice of \cite[p. 299]{Goodfellow-et-al-2016} \tabularnewline
\hline
Bias initialization & 0 & Follows advice of \cite[p. 299]{Goodfellow-et-al-2016} \tabularnewline
\hline
%Learning rate schedule & $\eta_{e}=\eta_{1}/(1+e)$ for epoch $e$ & Follows advice of \cite[p. 291]{Goodfellow-et-al-2016}  \tabularnewline
%\hline
Classification hidden layers (unless specified) & 4 & Table 2 of \cite{klambauer2017self} shows that most neural networks architectures performed well with 6 layers on the UCI datasets \tabularnewline
\hline
RNN hidden units & 300 & \cite{pascanu2013difficulty} use between 200-500 hidden units and \cite{klambauer2017self} use \{256, 512, 1024\}. 500 hidden units is consistent with both. \tabularnewline
\hline
Layer form & Rectangular (i.e. number of hidden units the same in each layer) & \cite{klambauer2017self} use this layer form \tabularnewline
\hline
Train-test split & 80\%-20\% & Follows advice of \cite[p. 119]{Goodfellow-et-al-2016} \tabularnewline
\hline
Mini-batch size & 100 & 100 is a common size according to \cite[p. 276]{Goodfellow-et-al-2016} \tabularnewline
\bottomrule
\end{tabular}
\end{table}

%Overall our results, IB outperforms EB in nearly all our experiments. The extent depends on the architecture. Shallow classification with enough grid points similar. However if few grid points and RNN architecture ... best.

% Recommendation!
%Nevertheless, it is our view that IB makes a better default method than EB for neural network problems, even for classification problems, where the performance of this method at worst matches EB and at best significantly outperforms it. In general.


%If we instead look at the second best learning rate, the average difference in accuracy of IB over EB increases to $0.65\%$, demonstrating its greater robustness to the learning rate.

%The goal is to simulate how a practitioner would approach the problem: by taking a grid search over a wide range of learning rates,
%running each algorithm for $10$ epochs, and using the model that has the
%lowest training error on the test set. We see that the performance of IB
%and EB are very similar, with the mean difference in test set
%classification accuracy being only $0.13\%$ higher for IB than EB. 


%Our final experiment tests the ability of EB and
%IB to train neural networks on $121$ classification experiments from the UCI
%database. The goal is to simulate how a practitioner would approach the
%problem: by taking a grid search over a wide range of learning rates,
%running each algorithm for $10$ epochs, and using the model that has the
%lowest training error on the test set. We see that the performance of IB
%and EB are very similar, with the mean difference in test set
%classification accuracy being only $0.13\%$ higher for IB than EB. 

% (with a
%standard deviation of $4.56$\%). This shows that even though IB might have
%better performance for higher learning rates, it is often the case that
%optimal performance is achieved with learning rates small enough for EB
%and IB to have similar performance. This can also be seen in Figures
%\ref{fig:main_results_no_clipping} and
%\ref{fig:main_results_with_clipping}. 

%When we thin the grid of learning rates to exclude the best learning rate, test robustness. Increase 5 fold to $0.65\%$.


%--------------------------------------------------
\section{Implementation within gradient framework with computational stability}
In most neural network codebases, such as PyTorch or Tensorflow, gradients $\nabla \ell_i (\theta^{(t)})$ are passed into an optimizer which takes the step $\theta^{(t+1)} = \theta^{(t)} - \eta \nabla \ell_i (\theta^{(t)})$. In order for ISGD to fit into such a framework it will be necessary to pass the gradient $\nabla \ell_i (\theta^{(t+1)})$ into an optimizer which takes the step $\theta^{(t+1)} = \theta^{(t)} - \eta \nabla \ell_i (\theta^{(t+1)})$.

The equations derived in Section~\ref{sec:ISGD_updates} show how to derive $\theta^{(t+1)}$ from $\theta^{(t)}$ using ISGD:
\begin{equation*}
\theta_{kj}^{(t+1)}  = \frac{\theta^{(t)}_{kj}}{1+\eta\mu} 
+ \alpha^{ki}_j\delta^{ki}_j\frac{z^{ki}(\theta^{(t)})}{\|z^{ki}(\theta^{(t)})\|_2^2}
\end{equation*}
for 
\begin{equation*}
\alpha^{ki}_j = \argmin_{\alpha}\left\{s^{ki}_j\cdot \sigma\left(\alpha \delta^{ki}_j + c^{ki}_j \right) + \alpha^2/2 \right\},
\end{equation*}
where $s^{ki}_j = \mbox{sign}(b^{ki}_j(\theta^{(t)}))$, $\delta^{ki}_j = \|z^{ki}(\theta^{(t)})\|_2\sqrt{\frac{\eta |b^{ki}_j|}{1+\eta\mu}}$ and $c^{ki}_j = \frac{\theta^{(t)\top}_{kj} z^{ki}(\theta^{(t)})}{1+\eta\mu}$. 
The gradient is thus
\begin{align*}
\nabla \ell_{ik} (\theta^{(t+1)}) &= \frac{\theta^{(t)}_{k} -\theta_{k}^{(t+1)}}{\eta}\\
&= \theta_{k}^{(t)}\frac{\mu}{1+\eta\mu} - \frac{(\alpha^{ki}(\theta^{(t)})\circ \delta^{ki}(\theta^{(t)})) z^{ki}(\theta^{(t)})^\top}{\eta\|z^{ki}(\theta^{(t)})\|_2^2}.
\end{align*}
where $\circ$ denotes the element-wise product. If $\eta$ is small then the division by $\eta$ in the second term can lead to computational rounding error issues. To avoid this, we reparameterize $u^{ki}(\theta^{(t)}) = - \frac{(\alpha^{ki}(\theta^{(t)})\circ \delta^{ki}(\theta^{(t)}))}{\eta\|z^{ki}(\theta^{(t)})\|_2^2}$. The gradient becomes
\begin{equation}\label{eq:stable_grad_update}
\nabla \ell_{ik} (\theta^{(t+1)}) = \theta_{k}^{(t)}\frac{\mu}{1+\eta\mu} + u^{ki}(\theta^{(t)})z^{ki}(\theta^{(t)})^\top
\end{equation}
for 
\begin{equation}\label{eq:u_update}
u^{ki}_j(\theta^{(t)}) = \argmin_u \left\{b^{ki}_j(\theta^{(t)})\cdot \sigma\left(c^{ki}_j - u \eta\|z^{ki}(\theta^{(t)})\|_2^2 \right) + \eta(1+\eta\mu) \|z^{ki}(\theta^{(t)})\|_2^2 \frac{u^2}{2} \right\},
\end{equation}
As (\ref{eq:stable_grad_update}) no longer divides by $\eta$ it will be far more computationally stable. It may be necessary to divide by $\eta$ when solving for $u$ in \ref{eq:u_update}, but typically the $\eta$ factors cancel out. The error in the ISGD gradient can be measured by comparing its gradient to the ESGD update when $\eta = 0$, for which the ISGD and ESGD gradients are equal. The stabilized ISGD gradients decrease the rounding errors from about $10^{-6}$ to $10^{-12}$. Below are the updates for the relu and arctan activation functions using $u$. As before, we will drop the superscripts and subscripts since they are clear from the context and will provide solutions to  
\begin{equation}\label{eq:u_update_no_scripts}
u^\ast = \argmin_u \left\{b\cdot \sigma(c - u \eta\|z\|_2^2) + \eta(1+\eta\mu) \|z\|_2^2 \frac{u^2}{2} \right\},
\end{equation}

%--------------------------------------------------
\subsection{Relu update with $u$}
Like in Section \ref{sec:Relu_alpha}, for $sgn(b)=+1$ there are three cases:
\begin{align*}
u^\ast = \begin{cases}
0 &\mbox{if }c\leq 0 \\
\frac{c}{\eta \|z\|_2^2} &\mbox{if }0< c\leq \eta \|z\|_2^2\frac{b}{1+\eta\mu} \\
\frac{b}{1+\eta\mu} &\mbox{if } c > \eta \|z\|_2^2\frac{b}{1+\eta\mu}
\end{cases}
\end{align*}
The middle case where $u^\ast =\frac{c}{\eta \|z\|_2^2}$ looks like it may be numerically unstable due to dividing by $\eta$. However in this case $u^\ast \leq \frac{b}{1+\eta\mu}$, and so the update is stable.

For $sgn(b)=-1$ there are two cases:
\begin{align*}
u^\ast = \begin{cases}
0 &\mbox{if } c\leq \frac{1}{2}\eta \|z\|_2^2\frac{b}{1+\eta\mu} \\
\frac{b}{1+\eta\mu} &\mbox{if } c > \frac{1}{2}\eta \|z\|_2^2\frac{b}{1+\eta\mu}.
\end{cases}
\end{align*}

%--------------------------------------------------
\subsection{Arctan update with $u$}
Like in Section \ref{sec:arctan_alpha} the arctan update can be written as a cubic equation:
\begin{equation*}
 u^3(\eta^2\|z\|_2^4)+ u^2 (-2c\eta\|z\|_2^2)  + u(1+c^2)   + (- \frac{b}{1+\eta\mu}) = 0
\end{equation*}
and can be solved using standard routines. Recall from Section \ref{sec:arctan_alpha} that there will either be one or three real solutions, and ISGD always uses the real solution that is closest to zero.



%There are other non-trust region methods that can add higher order information to backpropagation. Adaptive learning rate methods, like Adam \cite{kingma2014adam} and Adagrad \cite{duchi2011adaptive}, estimate appropriate per-parameter learning rates and momentum accelerates SGD in a common direction of descent \cite{zhang2017yellowfin}. Although these methods are useful if the loss surface is relatively smooth, they do not much help with cliff problems. 

%Numerous methods in the literature that have been proposed to add higher order information into ESGD. Adaptive learning rate methods, like Adam \cite{kingma2014adam} and Adagrad \cite{duchi2011adaptive}, estimate appropriate per-parameter learning rates and momentum accelerates SGD in a common direction of descent \cite{zhang2017yellowfin}. Although these methods are useful if the loss surface is relatively smooth, they do not much help with cliff problems. Instead the standard solution is to ``clip'' the gradients so that their magnitude is truncated at a pre-specified threshold \cite{pascanu2013difficulty}. Clipping has been shown to help deal with exploding gradients, but comes at the cost of sometimes suppressing beneficial large steps and the need to tune the clipping threshold parameter.



%Solving the trust region problem therefore has a similar complexity of solving the ISGD update, and so can only be approximately solved in neural network applications. 
%Another related set of algorithms is Hessian-Free methods \cite{martens2010deep,martens2011learning}, which can be thought of as optimizing a second order approximation to minibatch ISGD,
%\begin{equation*}
%\argmin_\theta \left\{2\eta \sum_{i\in\mathcal{M}}\ell_i(\theta)\!+\!\|\theta\!-\!\theta^{(t)}\|_2^2\right\}\!\approx\!\argmin_\theta \left\{\sum_{i\in\mathcal{M}}\nabla\ell_i(\theta)\!+\!(\theta\!-\!\theta^{(t)})^\top(G_\mathcal{M}\!+\!I/2\eta)(\theta\!-\!\theta^{(t)})\right\}
%\end{equation*}
%where $\mathcal{M}$ contains all points in the minibatch and $G_\mathcal{M} \approx \sum_{i\in\mathcal{M}}\nabla^2\ell_i(\theta)$ is the Gauss-Newton matrix. It has been demonstrated that Hessian-Free methods can make training more stable, which is what one would expect from an approximate ISGD method, but comes at a much higher per iteration cost than ESGD which offsets this benefit \cite{bengio2013advances}.

%Deterministic variants of ISGD were analyzed as early as the 1970s \cite{rockafellar1976monotone}. 
%ISGD is a stochastic version of this method that is designed to tackle large problems with additive optimization functions $\ell(\theta) = \frac{1}{N}\sum_{i=1}^N\ell_i(\theta)$. 

% Achieves the same loss with learning rates
%We empirically demonstrate that, compared to EB, IB manages to achieve lower losses for higher learning rates


%ISGD, like ESGD, proceeds by randomly sampling a datapoint $i$ and then updates $\theta$ as $\theta^{(t+1)} = \argmin_\theta \left\{2\eta_t \ell_i(\theta) + \|\theta - \theta^{(t)}\|_2^2\right\}$ where $\eta_t$ is the learning rate. 

Similar to standard SGD, ISGD is an iterative method that samples a random datapoint $i$ each iteration.  and, after solving an implicit gradient-like update equation, takes a step to decrease that datapoint's loss. 

%where  $\ell_i(\theta) = \ell_\theta(x_i,y_i)$ is the loss from datapoint~$i$.

%over a dataset $\mathcal{D}=\{(x_i,y_i)\}_{i=1}^N$,
%\begin{equation}\label{eq:loss_over_dataset}
%\ell(\theta) = \frac{1}{N} \sum_{i=1}^N \ell_i(\theta) + \frac{\mu}{2}\|\theta\|_2^2,
%\end{equation}

%\footnote{Note that we have overloaded the notation of $\ell(\cdot)$, which can refer to $\ell(\theta)$ as in (\ref{eq:loss_over_dataset}), $\ell(y, \cdot)$ or $\ell(\theta)=(\ell_1(\theta),...,\ell_N(\theta))$. Usually the interpretation is clear from the context, if not we indicate which interpretation to use.}
%Instead of optimizing (\ref{eq:loss_over_dataset}) using ESGD updates as is usually done, we will use an approximated ISGD. 


%Note that if we were to linearize the loss around the current iterate, $\ell_i(\theta) \approx \ell_i(\theta^{(t)}) + \nabla_\theta\ell_i(\theta)^\top (\theta - \theta^{(t)})$, then the ISGD and ESGD updates are equivalent. However if $\ell_i$ is not a linear function (and we don't linearize it) then the updates will be different. 

%From https://cs.stanford.edu/people/widom/paper-writing.html
%--------------------------------------------------
%\subsection{What is the problem? Why is it interesting and important?}

%However, an algorithm knowing where an optimum is and moving directly toward it, has never been achieved.

%This problem is exemplified by the \emph{exploding cliff}, illustrated in Figure~\ref{fig:cliff}. If an iterate is on the cliff face and standard backpropagation is used, then extremely large ``exploded'' gradient results in the next iterate moving far away from the global optimum at the foot of the cliff. 
%
%%----------
%\begin{figure}[h]
%\centering
%  \includegraphics[width=.45\linewidth]{plots/isgd_cliff}%isgd_cliff,  cliff
%\caption{Exploding gradient on a cliff face with Explicit and Implicit SGD steps. The arrow tail represents the current iterate and the head the next iterate. The figure is inspired by \cite[Fig. 6]{pascanu2013difficulty}.}\label{fig:cliff}
%\end{figure}
%%----------
%
%Ideally we would want a method that can identify the foot of the cliff as the lowest point on the loss surface and move directly there. In this paper we explore a method that can do this, called Implicit Stochastic Gradient Descent.\footnote{Implicit SGD comes in various forms under different names: Implicit SGD \cite{toulis2016implicit, toulis2015scalable, toulis2017asymptotic,toulis2016towards}, minibatch-prox \cite{wang2017memory}, generalized forward-backward splitting \cite{raguet2013generalized}, stochastic proximal iteration \cite{ryu2014stochastic},  stochastic proximal point algorithm \cite{patrascu2017nonasymptotic}, incremental proximal method \cite{bertsekas2011incremental} and incremental gradient method \cite{defazio2016simple}.}

\clearpage
Implicit SGD is contrasted from Explicit SGD (which for neural networks is another name for simple backpropagation) by its use of higher order information around the current iterate. The formulation of Implicit SGD is as follows. Let $\ell_i(\theta)$ represent the surface of the loss function of datapoint~$i$. In standard (explicit) SGD, we would update the iterate $\theta$ at time $t$ as $\theta^{(t+1)} = \theta^{(t)} - \eta_t \nabla_\theta \ell_i(\theta^{(t)})$, where $\eta_t$ is the learning rate. Implicit SGD has a similar form but takes the gradient at $\theta^{(t+1)}$ instead of $\theta^{(t)}$, that is, $\theta^{(t+1)} = \theta^{(t)} - \eta_t \nabla_\theta \ell_i(\theta^{(t+1)})$. This is equivalent to solving the Implicit SGD update equation,
\begin{equation}\label{eq:Implicit_SGD_formula}
\theta^{(t+1)} = \argmin_\theta \left\{2\eta_t \ell_i(\theta) + \|\theta - \theta^{(t)}\|_2^2\right\},
\end{equation}
which may also be thought of as a trust-region update. Note that if we were to make a first order approximation $\ell_i(\theta) \approx \ell_i(\theta^{(t)})+ \nabla \ell_i(\theta^{(t)})^\top (\theta - \theta^{(t)})$ in the Implicit SGD update, then the Implicit SGD update would become that same as Explicit SGD.

Let us return to the example where $\ell_i(\theta)$ is the cliff in Figure \ref{fig:cliff} with the iterate $\theta^{(t)}$ lying on the cliff face. It is clear from (\ref{eq:Implicit_SGD_formula}) that Implicit SGD would (with a sufficiently large learning rate) move directly to the foot of the cliff and not explode away from it. \emph{Implicit SGD is thus immune to the problem of exploding gradients}. Furthermore, Implicit SGD is known in convex optimization to be \emph{robust to the learning rate and unconditionally stable} \cite[Sec. 3.1]{toulis2015scalable} \cite[Sec. 5]{ryu2014stochastic}. By using higher order information Implicit SGD addresses two of the most important issues in neural network optimization: sensitivity to learning rates and immunity from exploding gradients \cite[Sec. 11.4.1]{Goodfellow-et-al-2016}.


%Arguably the most important hyperparameter is the learning rate \cite[Sec. 11.4.1]{Goodfellow-et-al-2016}. If it is too small then convergence will be too slow, but if it is too large then the algorithm may not converge at all. Large learning rates are particularly disastrous if paired with \emph{exploding gradients}, that is, points at which the gradient is orders of magnitude larger than usual. %In this case the resultant step (equal to the learning rate multiplied by the gradient) will be extremely large and may take the algorithm far away from any good values. 
%This is exemplified by the well known \emph{cliff problem}, illustrated in Figure \ref{fig:cliff}. If an iterate is on a cliff face, the extremely large ``exploded'' gradient results in an extremely large step size, taking the next iterate far away from the foot of the cliff. 


%--------------------------------------------------
%\subsection{Why is it hard? (E.g., why do naive approaches fail?)}
%The fundamental reason why neural network training is sensitive to the learning rate and exploding gradients is that they are typically trained using \emph{first order} Explicit Stochastic Gradient Descent (ESGD).\footnote{``Explicit'' SGD refers to vanilla SGD, to be contrasted with ``Implicit'' SGD which will be defined shortly.} The lack of higher order information makes these algorithms unable to know if taking a large step in a gradient descent direction will increase or decrease the objective. It does not know where the foot of the cliff is.

%--------------------------------------------------
%\subsection{Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)}
%Numerous methods in the literature that have been proposed to add higher order information into ESGD. Adaptive learning rate methods, like Adam \cite{kingma2014adam} and Adagrad \cite{duchi2011adaptive}, estimate appropriate per-parameter learning rates and momentum accelerates SGD in a common direction of descent \cite{zhang2017yellowfin}. Although these methods are useful if the loss surface is relatively smooth, they do not much help with cliff problems. Instead the standard solution is to ``clip'' the gradients so that their magnitude is truncated at a pre-specified threshold \cite{pascanu2013difficulty}. Clipping has been shown to help deal with exploding gradients, but comes at the cost of sometimes suppressing beneficial large steps and the need to tune the clipping threshold parameter.

%Adaptive learning rate methods, like Adam \cite{kingma2014adam} and Adagrad \cite{duchi2011adaptive}, estimate appropriate per-parameter learning rates and momentum accelerates SGD in a common direction of descent \cite{zhang2017yellowfin}.

%Neural networks, when well trained, have been shown to exhibit remarkable performance on a number of problem domains. However, training a neural networks is no simple task. Neural network training is highly sensitive to hyperparameter settings and the optimization algorithm used \cite{}. %Tuning hyperparameters and selecting the best optimization routine is often the most difficult and time-consuming process in applying deep learning models.


%The value of $\alpha$ is given by:
%\begin{align*}
%\alpha = \argmin_\alpha \sum_{m=1}^M &I\left[\left(\frac{\theta^{(t)\top} z}{1+\eta\mu} - B_{m+1}\right)\bigg/(\eta\|z\|_2^2)<  \alpha  \leq  \left(\frac{\theta^{(t)\top} z}{1+\eta\mu} - B_m\right) \bigg/ (\eta\|z\|_2^2)\right] \\
%&\cdot  \bigg[b\cdot \sigma_m\bigg(\frac{\theta^{(t)\top} z}{1+\eta\mu} - \alpha\cdot \eta\|z\|_2^2 \bigg) + \eta_t(1+\eta\mu) \|z\|_2^2 \frac{\alpha^2}{2}\bigg]
%\end{align*}



%The runtime difference between ESGD and ISGD is theoretically very similar if the input dimension $n$ and output dimension $m$ are relatively large. To see this, note that one forward and backwards pass through a layer requires three matrix vector products each with $nm$ multiplications and additions (one for the forward pass, one for the weight gradient and one for the backpropagated gradient). This is common to both ESGD and ISGD methods, and will typically be the dominant cost.
%
%ISGD has the extra expense of calculating $\|z\|_2^2$ at $2n$ flops and solving $m$ ISGD update equations on the backwards pass. The number of floating point operations (flops) required for solving the ISGD update equation depends on the activation function. For RELU, it requires no more than 10 flops, whereas arctan requires no more than 100 flops to solve the resulting cubic equation.
%
%Denote by $r$ the relative increase in runtime of ISGD over ESGD, i.e. $runtime(ISGD) \leq (1+r)\cdot runtime(ESGD)$. Then taking the above flop values as upper bounds on the ISGD update cost, we can upper bound $r$ as
%\begin{align*}
%r_{relu} &\leq \frac{2n + 10m}{3nm}\\
%r_{arctan} &\leq \frac{2n + 100m}{3nm}.
%\end{align*}
%We can substitute values of $n$ and $m$ from our experiments to get an idea of what relative difference in the runtimes we should expect. For the RNN music predictions the arctan activation function is used with $n,m=300$, and so $r\leq 11.33\%$. For the autoencoder we use the RELU activation function have values of $n,m=500$ for which $r \leq 0.8\%$. Thus, as claimed, the runtime gap between ESGD and ISGD should be small.

%\begin{align*}
%\alpha = \begin{cases}
%0 &\mbox{if }\theta^{\top} z\leq 0 \\
%\frac{\theta^{\top} z}{1+\eta\mu} \frac{1}{\eta \|z\|_2^2} &\mbox{if }0< \theta^{\top} z\leq \eta \|z\|_2^2b \\
%\frac{b}{1+\eta\mu} &\mbox{if } \theta^{\top} z > \eta \|z\|_2^2 b
%\end{cases}
%\end{align*}
%and when $sign(b)=-1$ there are two cases:
%\begin{align*}
%\alpha = \begin{cases}
%0 &\mbox{if } \theta^{\top} z\leq \frac{1}{2}\eta \|z\|_2^2b \\
%\frac{b}{1+\eta\mu} &\mbox{if } \theta^{\top} z > \frac{1}{2}\eta \|z\|_2^2b.
%\end{cases}
%\end{align*}

%\begin{align*}
%\alpha^\ast&=\argmin_\alpha\{s\cdot \sigma(\delta \alpha+c)+\alpha^2/2\}\\
%&= \argmin_\alpha\left\{\sum_{m=1}^MI[B^\ell_m\leq \delta \alpha+c < B^u_m]\left(s a_m(\delta \alpha+c)+s b_m+\alpha^2/2\right) \right\}.
%\end{align*}
%Let the minimal value of $\alpha$ restricted to the $m^{th}$ piece be denoted as
%\begin{align*}
%\alpha_m &= \argmin_\alpha\{s a_m(\delta \alpha+c)+s b_m+\alpha^2/2:~B^\ell_m\leq \delta \alpha+c < B^u_m\}\\
%&= 
%\begin{cases}
%-sa_m\delta &\mbox{if }B^\ell_m\leq c - sa_m\delta^2 < B^u_m\\
%\argmin_{\alpha\in\{(B^\ell_m-c)/\delta,(B^u_m-c)/\delta\}}\{s a_m(\delta \alpha+c)+s b_m+\alpha^2/2\} &\mbox{otherwise}
%\end{cases}
%\end{align*}
%and the piece which achieves the minimal value be denoted as
%\begin{equation*}
%m^\ast= \argmin_{m\in\{1,...,M\}}\{s a_m(\delta \alpha_m+c)+s b_m+\alpha_m^2/2\}.
%\end{equation*}
%It must be the case that $\alpha^\ast = \alpha_{m^\ast}$.



%Looking at the form of the derivative of $\arctan(x)$, it is natural to consider applying ISGD to functions with gradients of the form $\sigma'(x) = 1/ (1+|x|^k)$. The polynomial we need to solve would be of order $k+1$. Roots can only be analytically computed for $k=1,2,3$. For $k=1$ we have $\sigma(x) = \mbox{sign}(x)\cdot \log(1+|x|)$ which is a non-saturating sigmoidal-like function. When $k=3$ then $\sigma$ has some complicated sigmoidal form. Another interesting case is when $k\to\infty$ for which $\sigma(x)$ is the HardTanh function.


%--------------------------------------------------
\subsection{HardTanh}\label{sec:hardtanh}
The HardTanh function is a 3-piecewise-linear sigmoidal function
\begin{equation*}
\sigma(x) = 
\begin{cases}
-1 &\mbox{ if }x<-1\\
x &\mbox{ if }-1\leq x \leq 1\\
1 &\mbox{ if }x>1.
\end{cases}
\end{equation*}
It is sometimes used to back-propagate the signal in binarized neural networks \cite{hubara2016quantized}. Since HardTanh is an odd function $\argmin_{\alpha}\left\{s\cdot\sigma(\delta\alpha + c) + \alpha^2/2 \right\} = \argmin_{\alpha}\left\{\sigma(s\delta\alpha + sc) + \alpha^2/2 \right\}$ and so we do not have to do separate cases for $s=\pm 1$. The solution is:
\begin{align*}
\alpha^\ast = \begin{cases}
0 &\mbox{if } sc\leq -1 \mbox{ ~~~or~~~ } sc \geq 1+\frac{\delta^2}{2}\\
-s\delta &\mbox{if } \delta^2-1\leq sc \leq 1 \mbox{ ~~~or~~~ } \max\{1,\frac{\delta^2}{2}-1\}< sc < 1 + \frac{\delta^2}{2}\\
-\frac{1+sc}{s\delta} &\mbox{if } -1< sc< \min\{1,\delta^2-1\} \mbox{ ~~~or~~~ } 1< sc \leq \frac{\delta^2}{2}-1
\end{cases}
\end{align*}
Like for arctan, the HardTanh is non-convex and it is possible for there to be multiple optimal solutions. When $sc = 1+\frac{\delta^2}{2}$ there are two optimal values, $\alpha^\ast\in\{0,-s\delta\}$. By our simple rule, we take the optimal value to be $\alpha^\ast = 0$.




%In the first case $c$ is on the 0-flat part and is too far away from the hinge to move; and in the second part $c$ is either on the flat part and close to the hinge, or is on the slope. So ISGD takes a step even if it is on the flat part, as long as it is close enough to the hinge.



%$c = \frac{\theta^{(t)\top}_{kj} z^{ki}}{1+\eta_t\mu}$
%
%$c = \frac{\theta^{\top} z}{1+\eta\mu}$


%The first case corresponds to $c$ already lying on the 0-flat part of the RELU; the second to $c$ lying on the slope but close to the hinge and moving towards the hinge point; and the third case to lying on the slope far from the hinge. These updates are the same in ESGD, except that ESGD doesn't have the second case. As a result, ESGD overshoots the minimum at the hinge point.

\begin{equation*}
\theta_{kj}^{(t+1)}  \xrightarrow[]{\eta_t \to \infty} \argmin_{\alpha}\left\{s^{ki}_j\cdot \sigma\left(\alpha\cdot \|z^{ki}\|_2\sqrt{|b^{ki}_j|/\mu} \right) + \alpha^2/2 \right\}\cdot \sqrt{|b^{ki}_j|/\mu} \frac{ z^{ki}}{\|z^{ki}\|_2}
\end{equation*}
where we have used that $\delta^{ki}_j \to \|z^{ki}\|_2\sqrt{|b^{ki}_j|/\mu}$ and $c^{ki}_j \to 0$ as $\eta_t\to\infty$. 

%\begin{equation}\label{eq:theta_k_solution}
%\theta_{kj}^{(t+1)}  = \frac{\theta^{(t)}_{kj}}{1+\eta_t\mu} 
%+ \alpha^{ki}_j\delta^{ki}_j\frac{z^{ki}}{\|z^{ki}\|_2^2}
%\end{equation}




%\begin{equation}\label{eq:alpha_original}
%\alpha^{ki}_j = \argmin_{\alpha}\left\{s^{ki}_j\cdot \sigma\left(\alpha\cdot \delta^{ki}_j + c^{ki}_j \right) + \alpha^2/2 \right\},
%\end{equation}


%\begin{equation}\label{eq:alpha_original}
%\alpha^{ki}_j = \argmin_{\alpha}\left\{s^{ki}_j\cdot \sigma\left(\alpha\cdot \delta^{ki}_j + c^{ki}_j \right) + \alpha^2/2 \right\},
%\end{equation}




%\newsavebox{\mycasesx}% Store case "title" and brace
%\begin{align}
%  \sbox{\mycasesx}{$\displaystyle \alpha^\ast=\left\{\begin{array}{@{}c@{}}\vphantom{1\ x\geq0}\\\vphantom{0\ x<0}\end{array}\right.\kern-\nulldelimiterspace$\hspace{0.2em}}
%  \raisebox{-.5\ht\mycasesx}[0pt][0pt]{\usebox{\mycasesx}}
%     0 \quad \mbox{if } c\leq -\delta^2/2\tag{R4} \\
%     \delta \quad \mbox{if } c> -\delta^2/2\tag{R5}
%\end{align}



%% From https://tex.stackexchange.com/questions/31951/separate-labels-in-cases
%\newsavebox{\mycases}% Store case "title" and brace
%\begin{align}
%  \sbox{\mycases}{$\displaystyle \alpha^\ast =\left\{\begin{array}{@{}c@{}c@{}}\vphantom{1\ x\geq0}\\\vphantom{0\ x<0}\\\vphantom{0\ x<0}\\\vphantom{0\ x<0}\end{array}\right.\kern-\nulldelimiterspace$\hspace{0.25em}}
%  \raisebox{-.6\ht\mycases}[0pt][0pt]{\usebox{\mycases}}
%  0 \hspace*{2.6em} \mbox{if }c\leq 0\hspace*{2.25em}\tag{R1} \\
%  -c/\delta \quad \mbox{if }0< c\leq \delta^2\hspace*{0.0em}\tag{R2} \\
%  -\delta \hspace*{1,9em} \mbox{if }c > \delta^2\hspace*{1.85em}\tag{R3}
%\end{align}


%\begin{subnumcases}{\alpha^\ast = }
%   0 & if  $c\leq 0$ \label{positive}\\
%   -c/\delta & if  $0< c\leq \delta^2$ \label{positive}\\
%   -\delta & if  $c > \delta^2$ \label{negative}
%\end{subnumcases}





\textbf{ISGD in composite optimization}.  %\\
%\emph{How have people approached convex composite problems?}\\
The closest works to our own concern ISGD applied to optimization composite functions of the form $f(\theta) = \sum_{i=1}^Nh_i(c_i(\theta))$ where $h_i$ is closed convex and $c_i$ is smooth \cite{duchi2017stochastic, davis2017proximally}. The algorithm \cite{duchi2017stochastic} is similar to ours in that they linearize the one of the functions and iteratively optimize
\begin{align*}
\theta^{(t+1)} = \argmin_\theta \left\{2\eta_t h_i\left(c_i(\theta^{(t)}) + \nabla c_i(\theta^{(t)})^\top (\theta - \theta^{(t)})\right) + \|\theta - \theta^{(t)}\|_2^2\right\}
\end{align*}
where $i\in\{1,...,N\}$ is uniformly sampled. Convergence to stationary points is proven using nonconvex differential inclusions. Our proposed method can be thought of as an extension of their partial-linearization idea to functions with deep composition, i.e. $f = g^{(d)} \circ g^{(d-1)} \circ ...  \circ g^{(1)}$, where we linearize the outer ($h$), opposed to inner ($c$), function.

%--------------------------------------------------
\section{Literature review}
PUT THE REST OF THE LITERATURE REVIEW EITHER IN THE INTRODUCTION OR IN THE BEGINNING OF IMPLICIT BACKPROP SECTION.

Gradient-clipping solves the exploding gradient problem by truncating the magnitude of the gradient beyond a certain pre-specified value. Although this makes training more stable, it comes at the cost of using ``incorrect'' step-sizes\footnote{By ``incorrect'' we mean the step size is not equal to the theoretically derived step size that is the learning rate multiplied by the gradient.}. For activation functions like exponentials, ISGD can take ``correct'' step sizes that are smaller than gradient-clipped ESGD, and for hinged activation functions ISGD can have similar behavior to clipping. However for functions like the ReLU, ISGD step sizes may be large and gradient clipping could still be useful.

WRITE MORE ABOUT HOW GRADIENT NORM CLIPPING IS LIKE AN APPROXIMATE TRUST REGION METHOD. ISGD IS ALSO LIKE A TRUST REGION METHOD. WE WILL SEE IN THE EXPERIMENTS THAT THEY CAN BE USED ADDITIVELY TO GOOD EFFECT, ALTHOUGH THEIR INTERACTION IS NOT TRIVIAL.


\textbf{ISGD in ML applications.} % \\
%\emph{How has ISGD been used? Maybe I want to use it for an application and want to make sure it hasn't been done before.}\\


Methods like Adagrad learn the per-parameter learning rate over time and thereby take appropriate step sizes for each parameter which helps to make the algorithm more robust to the learning rate. Again such methods might be worth combining with ISGD updates.

%\textbf{Stable neural networks.}  %\\
%%\emph{How have people previously tried to make NN more stable?}\\
%Increasing the stability in training neural networks is a core area of neural network research. One approach is to make the architecture inherently stable by combining certain activation functions like in LSTMs \cite{hochreiter1997long} and residual neural networks \cite{he2016deep}, or designing stable activation functions like SELU \cite{klambauer2017self} and batch-normalization \cite{ioffe2015batch}. Another approach is to make the optimization more stable. Methods include gradient-clipping \cite{pascanu2013difficulty}, natural gradients \cite{desjardins2015natural}, Hessian-Free optimization \cite{martens2010deep,martens2011learning} and proximal methods like Adagrad \cite{duchi2011adaptive}. To our knowledge, the only place where implicit updates have been used in neural networks is as an activation function in the recently proposed variational networks \cite{kobler2017variational}. Indeed it was recently remarked in \cite{toulisstable} that ISGD had not yet been applied to neural networks and that its application is an interesting open research question.


%The idea of ISGD has been extended in a number of directions. Averaged ISGD was proposed in \cite{toulis2016towards, bertsekas2015incremental} and distributed ISGD with mini-batches was analysed in \cite{wang2017memory}. Accelerated deterministic proximal point methods for almost-convex optimization problems have been developed, which achieve near-optimal efficiency for convex problems yet also find stationary points for non-convex problems with a fast rate \cite{paquette2017catalyst, lin2017catalyst}.


%%\emph{Give an example}\\
%As an illustrative example of the differences between ISGD and ESGD, consider the quadratic function $f(\theta)=\theta^2/2$. The ESGD update is $\theta^{(t+1)} = \theta^{(t)}\cdot(1-\eta_t)$ whereas the ISGD update is $\theta^{(t+1)} = \theta^{(t)}/(1+\eta_t)$ where $\eta_t$ is the learning rate. The iterates of ESGD and ISGD for $\eta = 1.75$ are plotted in Figure~\ref{fig:SGD_vs_Implicit_SGD}. From the update equations it is clear that ISGD will converge for any value of $\eta>0$, whereas ESGD will only converge for $\eta<2$ and will diverge for $\eta>2$. For a more general discussion on the stability of ISGD vs ESGD see Section 3.2 of \cite{toulis2015scalable}.
%
%\begin{figure}
%\centering
%\begin{minipage}{.49\textwidth}
%  \centering
%  \includegraphics[width=.99\linewidth]{plots/SGD.pdf}
%\end{minipage}%
%\hfill
%\begin{minipage}{.49\textwidth}
%  \centering
%  \includegraphics[width=.99\linewidth]{plots/ISGD.pdf}
%\end{minipage}
%\caption{Illustration of the difference between ESGD and Implicit SGD in optimizing $f(\theta)=\theta^2/2$. The learning rate was set to be $\eta=1.75$ in both cases.}
%\label{fig:SGD_vs_Implicit_SGD}
%\end{figure}



%--------------------------------------------------
\subsection{What are the key components of my approach? Also include any specific limitations (and when proposing the idea, any potential difficulties).}
The key idea is to use Implicit Stochastic Gradient Descent (ISGD) for neural networks. ISGD cannot be naively applied, since the resultant implicit equations would be too hard to optimize. To make the optimization easier, we make two simplifications. Firstly the ISGD updates are done separately for each layer, keeping the parameters in the other layers constant. Secondly, when optimizing a layer, we linearize all higher layers and only keep the non-linearity in the layer being updated. These two assumptions are sufficient to make the updates tractable. Indeed, we will often be able to solve for the updates in closed form, making them no more expensive than ESGD.

\textbf{Limitations and difficulties}
\begin{itemize}
\item There is no guarantee that this method will be better in general.
\item The optimization will be slower each iteration, although for certain activation functions this will be negligible.
\item It is too difficult to solve the equations for a mini-batch. If a mini-batch is desired, then best to do ISGD updates separately for each data-point and then average the steps afterwards.
\end{itemize}

%More expensive methods include hessian-free \cite{martens2010deep,martens2011learning} and natural gradient \cite{desjardins2015natural} methods which directly estimate second order information. Although these methods help 


%Previous non-vanilla SGD method for neural networks include momentum methods (like Nesterov momentum) and per-parameter adaptive learning rate methods (like Adam).
%Momentum methods effectively learn curvature information as they progress, but have the disadvantage of potentially overshooting the optimum if the momentum rate(s) are not set correctly. Also, it takes a while to learn the curvature.
%Per-parameter adaptive learning rate methods learn the diagonal of the Hessian to have an appropriate step size for each parameter. 

%Neither of these methods help for instance if we have a sigmoidal activation with a large learning rate. Even though most of the time the step size will be small, if for a particular datapoint the parameters sit in the middle of the sigmoid where the gradient is largest, then the size size could be disproportionately large. The reason why these methods cannot help here is because they have little information about the gradient at points close by. The essential contribution of our method is that it does have access to this information, which should help convergence.
%
%The most popular methods for dealing with exploding/vanish gradients are batch-normalization and gradient clipping. Batch normalizing does an ``internal covariate shift'' to keep the gradients bounded. Its disadvantages is that it is expensive, batch-sensitive and distorts the ``true'' architecture. Gradient clipping clips the gradients to make them bounded. It has the disadvantage of corrupting the true gradient.


%Since neural networks typically have a very large number of parameters, they are typically fit with stochastic first order methods. As a result, they do not have access to curvature information at any particular point. A major consequence of this is that there is little information for choosing the step length (or equivalently, the learning rate). As a result, the methods are highly sensitive to the choice of learning rate.

%Many activation functions are flat except for a small domain where the gradient is quite steep, e.g. tanh. This is necessary to have hard decision boundaries, approximating a step function. The magnitude of the gradient in back-propagation is amplified by the number of layers. Dependent on the current parameters, the gradients can become either vanish (all layers flat) or explode (all layers steep). Since first order methods only look at the gradient at the current iterate value, it cannot perturb the iterate to a flatter region with a smaller, yet just as valid, gradient.

%The high level problem is: how to efficiently optimize neural networks? Neural networks are expensive to train and can be \textbf{sensitive to the learning rate}. They also suffer from the \textbf{exploding/vanishing} gradients for saturating activation functions. The challenge is to design a SGD method for neural networks that is robust to the learning rate, does not suffer from exploding/vanishing gradients and has fast convergence.

%Our numerics focus on the performance of ESGD and ISGD in just the first few epochs. 

%The reason is that instability is most likely to present itself within the early epochs when the learning rate is highest. Also if a typical decreasing learning rate schedule is used then the learning rate will decrease each epoch, making ESGD and ISGD perform more similarly. Thus the differences between the methods will exhibit themselves in the earlier epochs (when the learning rate is high), opposed to later epochs (when the learning rate is low).

\subsection{Datasets}
Four different types of datasets will be used to test different aspects of ISGD.
\begin{enumerate}

\item \textbf{Toy RNN.}  In the seminal LSTM \cite{hochreiter1997long} paper a number of challenging toy examples were proposed to test the performance of RNNs on long time series, where information at the beginning of the time series is relevant to the final prediction. These problems have subsequently become a standard measure \cite{martens2011learning, pascanu2013difficulty}. We we adopt precisely the same experimental setup of these problems as in \cite{pascanu2013difficulty}.

\item \textbf{Real world RNN: Polyphonic music prediction.} Following \cite{pascanu2013difficulty} we also measure the performance of RNNs on three music prediction tasks. We use the Piano-midi.de, Nottingham, MuseData and JSB Chorales datasets, as described in \cite{boulanger2012modeling}.

\item \textbf{Classification.} We draw on the experiments of \cite{klambauer2017self} and \cite{kiros2013training} for our general classification experiments. From \cite{kiros2013training} we draw on the MNIST dataset and use their same architecture. We also add in the Fashion MNIST dataset, which is more challenging, with the same architecture as MNIST. \cite{klambauer2017self} use 121 UCI classification datasets in their experiments.

\item \textbf{Autoencoder.} Like for classification, we take the MNIST and Fashion MNIST datasets and train an autoencoder as done in \cite{kiros2013training}.

\end{enumerate}


%All of these questions are interconnected. For example, robustness to learning rates would enable smaller (larger) learning rates to offset exploding (vanishing) gradients respectively. 
To address the exploding/vanishing gradients question we will focus most of our experiments on long RNN and deep DNN problems \footnote{Since ISGD for CNNs is computationally very expensive, we will not use any CNNs in our experiments. Note that it is possible to combine ESGD for the CNN layers with ISGD for the non-CNN layers, but we leave this investigation to future work.} On each problem we will measure the speed of convergence on the train, validate and test sets each epoch. To address the third question, multiple learning rates will be tried for each problem.

%--------------------------------------------------
\section{Softmax derivation}
The stochastic function for a single datapoint and single class is
\begin{align*}
f_{ik}(u,W) & = N(u_i + e^{-u_i}+(K-1)e^{x_i^\top (w_k - w_{y_i})-u_i}).
\end{align*}
Below we show how to solve the ISGD equations for $u$ and $W$ separately.

%--------------------------------------------------
\subsection{$u_i$ update}
We seek to solve
\begin{align*}
\min_{u_i}\{ 2\eta N(u_i + (1+(K-1)e^{x_i^\top (w_k - w_{y_i})})e^{-u_i}) + (u_i-\tilde{u}_i)^2\}
\end{align*}
Setting the derivative of $u_i$ equal to zero and dividing by 2,
\begin{align*}
0 = \eta N - b_i e^{-(u_i-\tilde{u}_i +\eta N)} + u_i-\tilde{u}_i
\end{align*}
where $b_i = \eta N(1+(K-1)e^{x_i^\top (w_k - w_{y_i})})\exp^{-\tilde{u}_i + \eta N}$. Letting $\delta_i = u_i-\tilde{u}_i + \eta N$, we observe that $\delta_i e^{\delta_i} = b_i$, which has solution $\delta_i = P(b_i)$ where $P$ denotes the principle branch of the Lambert-W function. Hence the solution is $u_i = \tilde{u}_i - \eta N + P(\eta N(1+(K-1)e^{x_i^\top (w_k - w_{y_i})})\exp^{-\tilde{u}_i + \eta N})$.

%--------------------------------------------------
\subsection{$w$ update}
Refer to Appendix F.1 of the ``Unbiased scaled softmax optimization'' paper. The solution is 
\begin{align*}
w_{y_i} & = \tilde{w}_{y_i} +a \frac{x_i}{2\|x_i\|_2^2}\\
w_k & = \tilde{w}_k - a \frac{x_i}{2\|x_i\|_2^2} 
\end{align*}
where
\begin{align}
a(u_i) &= P(2\eta N (K-1)\|x_i\|_2^2e^{x_i^\top (\tilde{w}_k - \tilde{w}_{y_i})-u_i})\nonumber\\
&= P(e^{x_i^\top (\tilde{w}_k - \tilde{w}_{y_i})-u_i + \log(2\eta N (K-1)\|x_i\|_2^2)}).\label{eq:a_u_function}
\end{align}



It will be convenient to reparameterize $v = u \eta\|z\|_2^2$ for which the update becomes
\begin{equation*}
v(1+(c - v)^2) = b'
\end{equation*}
where $b' = \frac{\eta\|z\|_2^2 b}{1+\eta\mu}$. The three roots of this equation are
\begin{align*}
v_1^\ast &= \frac{\beta}{3\sqrt[3]{2}} -\frac{\sqrt[3]{2}(3-c^2)}{\beta} + \frac{2c}{3} \\
v_2^\ast &= \frac{(1-i\sqrt{3})\beta}{6\sqrt[3]{2}} + \frac{(1+i\sqrt{3})(3-c^2)}{3\cdot  2^{2/3}\beta} + \frac{2c}{3}\\
v_3^\ast &= \frac{(1+i\sqrt{3})\beta}{6\sqrt[3]{2}} + \frac{(1-i\sqrt{3})(3-c^2)}{3\cdot  2^{2/3}\beta} + \frac{2c}{3}
\end{align*}
where $i = \sqrt{-1}$ is an imaginary number and 
\begin{align*}
\Delta &= 27b'^2 - 4b'c^3-36b'c+4c^4+8c^2+4\\
\gamma &= 27b' -2c^3-18c\\
\beta &= \sqrt[3]{3\sqrt{3\Delta} + \gamma}.
\end{align*}
It will often be the case that $\Delta \geq 0$ in which case $v_1^\ast$ is the only real root and should be chosen for the ISGD update. However it is possible that all three roots are real (e.g. $c=10$, $b'=50$).


Before we move onto the cases below, note that it is also possible to do ISGD updates for layers that share weights, for example Convolutional Neural Networks (CNNs). The problem is the updates tend to be far more complex and expensive to compute. In Appendix \ref{app:CNNs} we derive the ISGD updates for CNNs with max-pooling and linear activations, and show them to be equivalent to a linear-constrained quadratic program.




%The update equations for a CNN with RELUs and Max-pooling can be represented as a quadratic program and solved as such. Consider layer $k$ of width $w_k$ with one filter. The update equations can be written as
%\begin{align*}
%\min_\theta\{2\eta\sum_{i=1}^d a_k^{(i)}g_k^{(i)}(\theta) + \|\theta - \tilde{\theta}\|_2^2\}
%\end{align*}
%where $a_k^{(i)}\in\mathbb{R}$ are from the gradients of higher layers via the chain rule, $g_k^{(i)}(\theta) = \max\{[\theta^\top X_k^{(i)} + B_k^{(i)}]_+\}$ and $X_k^{(i)}, B_k^{(i)}$ are matrices. We can rewrite the equations as a QP:
%\begin{align*}
%\min_\theta &~~2\eta\sum_{i=1}^d a_k^{(i)}g_k^{(i)} + \|\theta - \tilde{\theta}\|_2^2\\
%s.t. & ~~g_k^{(i)}\geq h_{k,j}^{(i)}\qquad \forall j \\
%& ~~h_{k,j}^{(i)}\geq \theta^\top X_k^{(i)} + B_k^{(i)}\\
%& ~~h_{k,j}^{(i)}\geq 0
%\end{align*}
%Note that we would change the signs in the s.t. if $a_k^{(i)}<0$
%
%CNNs reduce to solving a quadratic program with linear constraints, the same setup as in OptNet \cite{amos2017optnet}.


%--------------------------------------------------
\subsection{Binary step}
The odd binary step function is $\sigma(x) = 2I[x\geq 0] -1$. The solution is
\begin{equation*}
\alpha^\ast = \begin{cases}
0 &\mbox{if } sc\leq 0 \mbox{ ~~~or~~~ } sc \geq 2|\delta|\\
-\frac{c}{\delta} &\mbox{if } sc < 2|\delta|.
\end{cases}
\end{equation*}

%--------------------------------------------------
\subsection{Parameteric rectified linear unit (PRELU)}
The PReLU function with parameter $\beta\geq 0$ is 
\begin{equation*}
\sigma(x) = 
\begin{cases}
\beta x &\mbox{ if }x<0\\
x &\mbox{ if } x \geq 0.
\end{cases}
\end{equation*}
There are different updates depending on $s$ and whether $\beta<1$ or $\beta\geq1$. \\
For $s=+1, \beta<1$:
\begin{equation*}
\alpha^\ast = \begin{cases}
- \delta \beta &\mbox{if } c\leq \beta\delta^2\\
-\frac{c}{\delta} &\mbox{if } \beta\delta^2 \leq c\leq \delta^2\\
-\delta &\mbox{if } c\geq \delta^2.
\end{cases}
\end{equation*}
For $s=+1, \beta\geq 1$:
\begin{equation*}
\alpha^\ast = \begin{cases}
-\delta \beta &\mbox{if } c< \beta\delta^2\\
-\delta &\mbox{if } c\geq \beta\delta^2.
\end{cases}
\end{equation*}
For $s=-1, \beta<1$:
\begin{equation*}
\alpha^\ast = \begin{cases}
\delta \beta &\mbox{if } c\leq -\frac{\delta^2}{2}\\
\delta &\mbox{if } c> -\frac{\delta^2}{2}.
\end{cases}
\end{equation*}
For $s=-1, \beta\geq1$:
\begin{equation*}
\alpha^\ast = \begin{cases}
\delta\beta &\mbox{if } c\leq-\delta^2\beta\\
-\frac{c}{\delta} &\mbox{if } -\delta^2\beta\leq c\leq -\delta^2\\
\delta &\mbox{if } c\geq -\delta^2.
\end{cases}
\end{equation*}


%--------------------------------------------------



which is exactly the activation function used to back-propagate the signal in binarized NNs, called "HardTanh". For ISGD we would then have $w = O(1)$. If we consider $\sigma(aw)$ then the update is
\begin{align*}
w = 
\begin{cases}
\tilde{w} & \mbox{ if }a\tilde{w} \leq -1
\mbox{~~~or~~~} 
a\tilde{w}  \geq 1+ a^2\eta/2\\
\tilde{w}-a\eta & \mbox{ if } \max\{1,-1+a^2\eta\} \leq a\tilde{w}  \leq 1+ a^2\eta/2
\mbox{~~~or~~~}
-1+a^2\eta \leq a\tilde{w}  \leq 1\\
-1/a & \mbox{ if } 1 \leq a\tilde{w} \leq \min\{1+ a^2\eta/2, -1+a^2\eta\}
\mbox{~~~or~~~}
-1 \leq a\tilde{w} \leq \min\{1, -1+a^2\eta\}
\end{cases}
\end{align*}
Note that such a neural network is provably stable. For $w = \tilde{w}-a\eta$ we have $a^2\eta \leq 4$ or $a\leq 2\eta^{-1/2}$ for both of the conditions to be potentially valid. Thus the step size is at most $a\eta = 2\eta^{1/2}$. For the second case of $w = -1/a$ we have
\begin{align*}
\tilde{w} - w & = \frac{1}{a}((a\tilde{w}) - (aw))\\
& = \frac{1}{a}((a\tilde{w}) + 1)\\
& \leq \frac{1}{a}(\min\{1, -1+a^2\eta\} + 1)\\
& = \min\{2/a, a\eta\}\\
& \leq \sqrt{2}\eta^{1/2}
\end{align*}
where the last inequality comes from maximizing over $a$. So again we find the same upper bound on the step size of $2\eta^{1/2}$. However for the first case of $w = -1/a$ we have only that the step is bounded by $a\eta$ without any condition on $a$. This could for example occur when $w=a\eta/2$ and $a$ is very large. Note that ISGD has allowed the algorithm to move even when it is on the flat part of $\sigma$.

This activation function also has the benefit of binarization and sparsity.

Binary literature: \cite{hubara2016quantized, yin2016quantization, courbariaux2015binaryconnect}

%--------------------------------------------------
\section{Choices in NN-ISGD}
%--------------------------------------------------
\subsection{Backprop gradients}
Use implicit or explicit gradients to backprop? Shouldn't make a difference in the proof.

%--------------------------------------------------
\subsection{RNNs}
In RNNs the same parameters are used recurrently. A natural solution is to first update $\theta$ using the function from the last occurrence (acting like the input to the last occurrence is fixed), then update $\theta$ using the function from the second last occurrence (acting like the input to the second last occurrence is fixed and linearizing the last occurance),... until the final occurrence. This hack should be ok, but isn't satisfying as changing $\theta$ should change the values in all layers.

%--------------------------------------------------
\subsection{Ordering of parameter updates}
Order the parameter updates as $\theta_d, \theta_{d-1},...\theta_1$ and use the new value of $\theta_d, \theta_{d-1},...\theta_{k+1}$ when updating $\theta_k$. Since ISGD has smaller gradients, this ensures that the product of the gradients is small! This should help solve the exploding gradient problem.

Note that this idea can also be applied with vanilla SGD. It will generally be the case for both vanilla and implicit SGD that the gradient will be smaller at the new iterate value (this is exactly what gradient descent is about --- converging to a zero gradient!). So the ordering of updates is a secondary contribution that may already exist in the literature.

Note that doing this might be dodgy in that the back-propagation does not correspond to the forward propagated value if the parameters have changed in the upper layers. So perhaps this isn't a good idea.

\begin{proof}[Proof of Theorem \ref{thm:main}]
Let $P$ denote the projection and $\ell$ the loss over all datapoints. From Lemma \ref{lm:nabla_f_g_bound} we know there exists a $\bar{\eta}_C>0$ and $d_{\bar{\eta}_C}>0$ such that for all $0<\eta<\bar{\eta}_C$ and $\theta\in C$ we have $\|\nabla \ell_i(\theta) - g_i(\theta^{(t)};\eta)\|_2 \leq d_{\bar{\eta}_C}\eta$.
\begin{align*}
\mathbb{E}[\ell(\theta^{(t+1)})] &= \mathbb{E}[\ell(P(\theta^{(t)}) - \eta_t g_i(\theta^{(t)};\eta_t))] \\
&\leq \mathbb{E}[\ell(\theta^{(t)}) - \eta_t g_i(\theta^{(t)};\eta_t)] \\
&= \mathbb{E}[\ell(\theta^{(t)}) - \eta_t g_i(\theta^{(t)};\eta_t)^\top \nabla \ell(\theta^{(t)}) + \eta_t^2 g_i(\theta^{(t)};\eta_t)^\top \nabla^2 \ell(\theta^{(t+1/2)})g_i(\theta^{(t)};\eta_t)]
\end{align*}
where $\theta^{(t+1/2)}$ is some convex combination of $\theta^{(t)}$ and $\theta^{(t+1)}$. 
From Lemma \ref{lm:bound_inner_product} we know that $g_i(\theta^{(t)};\eta_t)^\top \nabla \ell(\theta^{(t)}) \geq \nabla \ell_i(\theta^{(t)})^\top \nabla \ell(\theta^{(t)}) - d_{\bar{\eta}_C}\eta_t\|\nabla \ell(\theta^{(t)})\|_2$. 

\begin{align*}
&\mathbb{E}[\ell(\theta^{(t+1)})] \\
&\leq \mathbb{E}[\ell(\theta^{(t)})] - \eta_t\mathbb{E}[\nabla \ell_i(\theta^{(t)})^\top \nabla \ell(\theta^{(t)})]  \\
&~~~~~+ \eta_t^2 \mathbb{E}[d_{\bar{\eta}_C}\|\nabla \ell(\theta^{(t)})\|_2^2 + g_i(\theta^{(t)};\eta_t)^\top \nabla^2 \ell(\theta^{(t+1/2)})g_i(\theta^{(t)};\eta_t)]\\
&\leq \mathbb{E}[\ell(\theta^{(t)})] - \eta_t(1-\eta d_{\bar{\eta}_C})\mathbb{E}[\|\nabla \ell(\theta^{(t)})\|_2^2] + \eta_t^2 B,
\end{align*}
where $B = \max_{i,\theta\in C,\eta<\bar{\eta}_C}\{g_i(\theta;\eta)^\top \nabla^2 \ell(\theta^{(+1/2)})g_i(\theta;\eta)\}$.
Summing over multiple iterations
\begin{align*}
\mathbb{E}[\ell(\theta^{(0)})-\ell(\theta^{(T+1)})] &= \sum_{t=1}^{T} \mathbb{E}[\ell(\theta^{(t)})-\ell(\theta^{(t+1)})]\\
&\geq \sum_{t=1}^{T} \eta_t\mathbb{E}[\|\nabla \ell(\theta^{(t)})\|_2^2] - \eta_t^2 B \\
&= \sum_{t=1}^{T} \eta_t\mathbb{E}[\|\nabla \ell(\theta^{(t)})\|_2^2] - B \sum_{t=1}^{T}\eta_t^2.
\end{align*}
By assumption $\sum_{t=1}^{T}\eta_t^2<\infty$. Also for any $T$ we have $\mathbb{E}[\ell(\theta^{(0)})-\ell(\theta^{(T+1)})] \leq \ell(\theta^{(0)}) -\min_{\theta}\{\ell(\theta)\} <\infty$. It follows that the sum $\sum_{t=1}^{\infty} \eta_t\mathbb{E}[\|\nabla \ell(\theta^{(t)})\|_2^2] $ must be finite. This implies that $\lim_{t\to\infty}\mathbb{E}[\|\nabla \ell(\theta^{(t)})\|_2^2] = 0$.

\end{proof}

%\begin{theorem}\label{thm:main}
%Assume there exists some convex set $C$ such that projecting $\theta$ onto $C$ always decreases the loss. Let the learning rate be such that $\sum_{t=1}^\infty \eta_t = \infty$ and $\sum_{t=1}^\infty \eta_t^2 < \infty$ with $\eta_t<\bar{\eta}_C$ for all $t$. Then $C$-projected NN-ISGD converges to a stationary point.
%\end{theorem}

%--------------------------------------------------
%\begin{lemma}\label{lm:bounded_theta}
%The optimal $\theta^\ast$ satisfies $\|\theta^\ast\|_2^2\leq \frac{2}{\mu}\ell(0)$.
%\end{lemma}
%
%\begin{proof}
%\begin{equation*}
%\frac{\mu}{2}\|\theta^\ast\|_2^2 \leq \ell(\theta^\ast) \leq \ell(0)
%\end{equation*}
%\end{proof}
%where in the first inequality we used the assumption that $\ell_\theta(x,y)\geq 0$. Rearranging yields the desired result.


%--------------------------------------------------
%\begin{lemma}\label{lm:nabla_f_g_bound}
%Let $g_i(\theta^{(t)};\eta)$ be the gradient used to take a step in NN-ISGD when datapoint $i$ is sampled, i.e. $\theta^{(t+1)} = \theta^{(t)} - \eta g_i(\theta^{(t)};\eta)$. Then for any convex set $C$ there exists a $\bar{\eta}_C>0$ and $d_{\bar{\eta}_C}>0$ such that for all $0<\eta<\bar{\eta}_C$ and $\theta\in C$ we have $\|\nabla \ell_i(\theta^{(t)}) - g_i(\theta^{(t)};\eta)\|_2 \leq d_{\bar{\eta}_C}\eta$.
%\end{lemma}
%
%\begin{proof}
%Statement is definitely true. Not sure what is the best method to prove.
%\end{proof}

%--------------------------------------------------
\subsection{Generic update equations with ridge regularization}
Let us add a ridge-regularization term $\frac{\mu}{2}\|\theta\|_2^2$ to the loss in (\ref{eq:ell_original}),
\begin{equation*}
\ell_\theta(x,y) =~ \ell(y, \cdot) \circ  f_{\theta_d}^{(d)} \circ f_{\theta_{d-1}}^{(d-1)} \circ ... \circ f_{\theta_1}^{(1)}(x) + \frac{\mu}{2}\|\theta\|_2^2.
\end{equation*}
The derivation for the ISGD updates is the same as in Section \ref{sec:generic_update} until line (\ref{eq:generic_update_line_common}) which for ridge-regularized losses is
\begin{align*}
&\min_{\theta^{(k)}_j}\left\{2\eta \left(g_j \sigma( \theta^{(k)\top}_j \bar{z}^{(k)})  + \frac{\mu}{2}\|\theta^{(k)}_j\|_2^2\right) + \|\theta^{(k)}_j - \tilde{\theta}^{(k)}_j\|_2^2 \right\}.
\end{align*}

It must be the case that $\theta^{(k)}_j = \tilde{\theta}^{(k)}_j + \alpha^{(k)}_j \frac{\bar{z}^{(k)}}{\|\bar{z}^{(k)}\|_2}$, since the first term only has the inner product $\theta^{(k)\top}_j \bar{z}^{(k)}$ and the second minimizes the distance from $\theta^{(k)}_j$ to $\tilde{\theta}^{(k)}_j$. The equation\footnote{If there are multiple solutions to $\alpha$ we take the value of $\alpha$ with zero gradient closest to $\alpha = 0$, i.e. $\alpha_j^{(k)} = \argmin_\alpha\{\alpha^2:~\nabla_\alpha (2\eta g_j \sigma(\tilde{\theta}^{(k)\top}_j \bar{z} +  \alpha \|\bar{z}\|_2) + \alpha^2)=0\}$. We assume that $\alpha_j^{(k)}$ is finite, which it will be for all of the activation functions we consider in this paper.} for $\alpha^{(k)}_j\in\mathbb{R}$ is
\begin{align*}
\alpha^{(k)}_j &= \argmin_{\alpha}\left\{2\eta g_j \sigma( \|\bar{z}^{(k)}\|_2\alpha + \tilde{\theta}^{(k)\top}_j \bar{z}^{(k)}) + \alpha^2 \right\}.
\end{align*}
With the transformation $\beta^{(k)}_j = \alpha^{(k)}_j/\sqrt{2\eta |g_i|}$ it further simplifies to
\begin{equation}\label{eq:beta_original}
\beta^{(k)}_j = \argmin_{\beta}\left\{s_i\cdot \sigma(\delta^{(k)}_j \beta + c^{(k)}_j) + \beta^2 \right\}.
\end{equation}
where $s_i=\mbox{sign}(g_i)\in\{-1,+1\}$,~ $c^{(k)}_j = \tilde{\theta}^{(k)\top}_j \bar{z}^{(k)}\in\mathbb{R}$ and $\delta^{(k)}_j = \sqrt{2\eta |g_i|}\|\bar{z}^{(k)}\|_2>0$. 




\subsection{Generic update equations}\label{sec:generic_update}
Let us now derive the ISGD updates for a generic layer $k$ with activation function $\sigma$. Let $\theta_k = (W^{(k)}, b^{(k)})\in \mathbb{R}^{D_{k+1} \times (1+D_k)}$ where $W^{(k)} \in \mathbb{R}^{D_{k+1} \times D_k}$ and $b^{(k)} \in \mathbb{R}^{D_{k+1}}$. Denote $z^{(k)} = f^{(k-1:1)}_{\theta_{k-1:1}}(x) \in \mathbb{R}^{D_{k}}$ and $g = \nabla \ell_{\tilde{\theta}_{d:k+1},y}^{(d:k+1)}\bigg|_{f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)} \in \mathbb{R}^{D_{k+1}}$. The output of the $k^{th}$ layer is thus $f_{\theta_{k}}^{(k)}(z^{(k)}) = \sigma(W^{(k)}z^{(k)} + b^{(k)})$ where $\sigma$ is applied element-wise.
Then the ISGD update equations are 
\begin{align*}
&\argmin_{\theta_k}\left\{2\eta (\ell_{\tilde{\theta}}(x,y) + g^\top( f_{\theta_{k}}^{(k)}(z^{(k)}) - f_{\tilde{\theta}_{k}}^{(k)}(z^{(k)}) ) + \|\theta_k - \tilde{\theta}_k\|_2^2 \right\}\\
&=\argmin_{\theta_k}\left\{2\eta g^\top f_{\theta_{k}}^{(k)}(z^{(k)}) + \|\theta_k - \tilde{\theta}_k\|_2^2 \right\}\\
&=\argmin_{W^{(k)}, b^{(k)}}\left\{2\eta g^\top \sigma(W^{(k)}z^{(k)} + b^{(k)}) + \|W^{(k)} - \tilde{W}^{(k)}\|_2^2 + \|b^{(k)} - \tilde{b}^{(k)}\|_2^2 \right\}\\
&=\argmin_{W^{(k)}, b^{(k)}}\left\{\sum_{j=1}^{D_{k+1}}2\eta g_j \sigma(W^{(k)\top}_j z^{(k)} + b^{(k)}_j) + \|W^{(k)}_j - \tilde{W}^{(k)}_j\|_2^2 + \|b^{(k)}_j - \tilde{b}^{(k)}_j\|_2^2 \right\}
\end{align*}
where $W^{(k)}_j \in\mathbb{R}^{D_k}$ is the $j^{th}$ row of $W^{(k)}$.
The minimization splits into separate minimization problems, one for each dimension.
\begin{align}
&\argmin_{W^{(k)}_j, b^{(k)}_j}\left\{2\eta g_j \sigma(W^{(k)\top}_j z^{(k)} + b^{(k)}_j) + \|W^{(k)}_j - \tilde{W}^{(k)}_j\|_2^2 + \|b^{(k)}_j - \tilde{b}^{(k)}_j\|_2^2 \right\}\nonumber\\
&=\argmin_{W^{(k)}_j, b^{(k)}_j}\left\{2\eta g_j \sigma( (W^{(k)}_j; b^{(k)}_j)^\top (z^{(k)};1)) + \|W^{(k)}_j - \tilde{W}^{(k)}_j\|_2^2 + \|b^{(k)}_j - \tilde{b}^{(k)}_j\|_2^2 \right\}\nonumber\\
&=\argmin_{\theta^{(k)}_j}\left\{2\eta g_j \sigma( \theta^{(k)\top}_j \bar{z}^{(k)}) + \|\theta^{(k)}_j - \tilde{\theta}^{(k)}_j\|_2^2 \right\} \label{eq:generic_update_line_common}
\end{align}
where $\theta^{(k)}_j = (W^{(k)}_j; b^{(k)}_j)\in \mathbb{R}^{1+D_k}$, $\bar{z}^{(k)} =(z^{(k)};1)\in \mathbb{R}^{1+D_k}$ and we use the MATLAB syntax of $(,)$ for appending columns and $(;)$ for appending rows. It must be the case that $\theta^{(k)}_j = \tilde{\theta}^{(k)}_j + \alpha^{(k)}_j \frac{\bar{z}^{(k)}}{\|\bar{z}^{(k)}\|_2}$, since the first term only has the inner product $\theta^{(k)\top}_j \bar{z}^{(k)}$ and the second minimizes the distance from $\theta^{(k)}_j$ to $\tilde{\theta}^{(k)}_j$. The equation\footnote{If there are multiple solutions to $\alpha$ we take the value of $\alpha$ with zero gradient closest to $\alpha = 0$, i.e. $\alpha_j^{(k)} = \argmin_\alpha\{\alpha^2:~\nabla_\alpha (2\eta g_j \sigma(\tilde{\theta}^{(k)\top}_j \bar{z} +  \alpha \|\bar{z}\|_2) + \alpha^2)=0\}$. We assume that $\alpha_j^{(k)}$ is finite, which it will be for all of the activation functions we consider in this paper.} for $\alpha^{(k)}_j\in\mathbb{R}$ is
\begin{align*}
\alpha^{(k)}_j &= \argmin_{\alpha}\left\{2\eta g_j \sigma( \|\bar{z}^{(k)}\|_2\alpha + \tilde{\theta}^{(k)\top}_j \bar{z}^{(k)}) + \alpha^2 \right\}.
\end{align*}
With the transformation $\beta^{(k)}_j = \alpha^{(k)}_j/\sqrt{2\eta |g_i|}$ it further simplifies to
\begin{equation}\label{eq:beta_original}
\beta^{(k)}_j = \argmin_{\beta}\left\{s_i\cdot \sigma(\delta^{(k)}_j \beta + c^{(k)}_j) + \beta^2 \right\}.
\end{equation}
where $s_i=\mbox{sign}(g_i)\in\{-1,+1\}$,~ $c^{(k)}_j = \tilde{\theta}^{(k)\top}_j \bar{z}^{(k)}\in\mathbb{R}$ and $\delta^{(k)}_j = \sqrt{2\eta |g_i|}\|\bar{z}^{(k)}\|_2>0$. 
Thus the ISGD update breaks down into $D_{k+1}$ separate one-dimensional optimization problems. The difficulty of solving the update depends on the function $\sigma$. An optimal $\alpha$ can always be computed using the bisection method, although this may be slow. There are certain important activation functions for which $\alpha$ has a closed form solution --- we explore these in the next section.




Let $\tilde{\theta}$ denote the current values of $\theta$. Consider a small perturbation in $\theta_k$. Using Taylor series expansions we can linearize the loss and layers $d:k+1$ as
\begin{align}
\ell_{\theta_k,\tilde{\theta}_{-k}} (x,y) =&~ \ell_{\tilde{\theta}}(x,y) +  \nabla \ell_{\tilde{\theta}_{d:k+1},y}^{(d:k+1)}\bigg|_{f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)} ^\top 
( f_{\theta_{k}}^{(k)}\circ f_{\tilde{\theta}_{k-1:1}}^{(k-1:1)}(x) - f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)) \label{eq:Taylor_series}\\
&~ + O(\|f_{\theta_{k}}^{(k)}\circ f_{\tilde{\theta}_{k-1:1}}^{(k-1:1)}(x) - f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)\|_2^2) \nonumber\\
=&~ \ell_{\tilde{\theta}}(x,y) +  \nabla \ell_{\tilde{\theta}_{d:k+1},y}^{(d:k+1)}\bigg|_{f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)} ^\top 
( f_{\theta_{k}}^{(k)}\circ f_{\tilde{\theta}_{k-1:1}}^{(k-1:1)}(x) - f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)) \nonumber\\
&~ + O(\|\theta_k - \tilde{\theta}_k\|_2^2) \nonumber
\end{align}
where the derivative $\nabla \ell_{\tilde{\theta}_{d:k+1},y}^{(d:k+1)}$ is taken with respect to its argument $f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)\in\mathbb{R}^{D_{k+1}}$, not $\theta_{d:k+1}$.

Instead of doing ISGD on $\ell_{\theta_k,\tilde{\theta}_{-k}}(x)$ we will do it on the truncated Taylor series expansion in (\ref{eq:Taylor_series}). 
\begin{align}
\ell_{\theta_k,\tilde{\theta}_{-k}} (x,y) =&~ \ell_{\tilde{\theta}}(x,y) +  \nabla \ell_{\tilde{\theta}_{d:k+1},y}^{(d:k+1)}\bigg|_{f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)} ^\top 
( f_{\theta_{k}}^{(k)}\circ f_{\tilde{\theta}_{k-1:1}}^{(k-1:1)}(x) - f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)) \label{eq:Taylor_series}\\
&~ + O(\|\theta_k - \tilde{\theta}_k\|_2^2) \nonumber
\end{align}


Note that if we had also linearized layer $k^{th}$ layer as
\begin{align*}
f_{\theta_{k}}^{(k)}\circ f_{\tilde{\theta}_{k-1:1}}^{(k-1:1)}(x) =  f_{\tilde{\theta}_{k:1}}^{(k:1)}(x) + \nabla_{\theta_{k}} f_{\theta_{k}, \tilde{\theta}_{k}}^{(k)}\bigg|_{\tilde{\theta}_k}  (\theta_k - \tilde{\theta}_k) + O(\|\theta_k - \tilde{\theta}_k\|_2^2),
\end{align*}
where $\nabla_{\theta_{k}} f_{\theta_{k}, \tilde{\theta}_{k}}^{(k)}\bigg|_{\tilde{\theta}_k} \in \mathbb{R}^{D_{k+1} \times P_k}$ then 
\begin{align*}
\ell_{\theta_k,\tilde{\theta}_{-k}} (x,y) =&~ \ell_{\tilde{\theta}}(x,y) +  \nabla \ell_{\tilde{\theta}_{d:k+1},y}^{(d:k+1)}\bigg|_{f_{\tilde{\theta}_{k:1}}^{(k:1)}(x)}  ^\top 
\nabla_{\theta_{k}} f_{\theta_{k}, \tilde{\theta}_{k}}^{(k)}\bigg|_{\tilde{\theta}_k}  (\theta_k - \tilde{\theta}_k) + O(\|\theta_k - \tilde{\theta}_k\|_2^2)
\end{align*}
and ISGD would be equivalent to ESGD. 


%--------------------------------------------------
\subsection{Illustration for sigmoid}
Let $\sigma(x)=\arctan(x)$ where $x\sim \mathcal{N}(0,\sigma^2)$. Also let $x^+$ denote the  ISGD update. When $\eta$ is large then $\mathbb{E}[\sigma'(x^+)]$ is small. It should also have lower variance that ESGD (explicit SGD). To illustrate this plot the mean and variance of $\sigma'(x^+)$ and $\sigma'(x)$ for increasing $\eta$. This should illustrate that ISGD is more robust to the learning rate and has lower variance. Do this for $\sigma^2 = 0.1, 1, 10$. Ironically when the learning rate is large, the probability of taking big steps is smaller!

\subsubsection{Sigmoid functions and Arctan}
For arctan $\sigma(w) = arctan(aw)$ with $a\geq 0$ the update equations reduce to the cubic:
\begin{align*}
0 &= -\eta a+(w-\tilde{w})((aw)^2+1)\\
w &= \tilde{w} + \eta\frac{  a}{(aw)^2+1}
\end{align*}
whereas for vanilla SGD it is $w = \tilde{w} + \eta\frac{  a}{(a\tilde{w})^2+1}$. Instead of solving the cubic using the cubic formula, it might be faster to have an approximate solution $v$ which we refine by repeatedly updating as $v^+ = \tilde{w} + \eta\frac{  a}{(av)^2+1}$ with an initial value of $v=\tilde{w}$. If $v = w +O(\eta^k)$, then 
\begin{align*}
v^+ &= \tilde{w} + \eta\frac{a}{(av)^2+1}\\
&= \tilde{w} + \eta\frac{a}{(aw +O(\eta^k))^2+1}\\
&= \tilde{w} + \eta\frac{a}{(aw )^2+1} + O(\eta^{k+1})
\end{align*}
and so the error decreases by a factor of $O(\eta)$ each iteration. If $\eta$ is small then only a small number of iterations would be required to converge. Since the numbers are small enough to be stored in the cache or low registers, it should be extremely fast to iterate. We could also use the bisection method.

If we include the back-propagated gradients as $r$ and denote $\gamma = r\eta$, then the update equations are
\begin{align*}
w &= \tilde{w} + \frac{\gamma a}{a^2w^2+1}
\end{align*}
We can show that $w = O((\gamma/a)^{1/3})$. The proof outline is 
\begin{align*}
w &\approx \frac{\gamma a}{a^2w^2}
\end{align*}
for large $w$, which has the solution $w = \gamma^{1/3}a^{-1/3}$. This should be contrasted to vanilla SGD which has $w = O(\gamma a)$. Note the inverse relation to $a$: vanilla SGD takes large steps, whereas ISGD takes small steps with large $a$! This significantly makes it much more difficult to have large step sizes. The only case where we can take large step sizes is if $\tilde{w}$ is very large and $a/\gamma$ very small (making the $\frac{\gamma a}{a^2w^2+1}$ term dominate).

We can generalize this to make large gradients even harder to achieve. Define $\sigma(x) = \int \frac{1}{|y|^3+1} dy$ for even $k$ with $\sigma(0)=0$ (so that the function is odd). Then we have $w = \gamma^{1/4}$. Note that the resulting solution for $w$ is a quartic that can be solved in closed form.

We can generalize this idea to different orders, but the problem is that $\sigma(x)$ might be expensive to compute, which is important for forward-propagation. We should be able to do back-propagation for any order $k$ assuming that the formula:
\begin{align*}
w &= \tilde{w} + \frac{\gamma}{|w|^k+1}
\end{align*}
is a contraction.

If we take $k=1$ then $\sigma(x) = sgn(x)\cdot\log(|x|+1)$. This has the interesting property that $w = O(\sqrt{\gamma})$ and is independent of $a$. The implicit update equations are just a quadratic, which are quick to solve. Note sure why $\sigma(x) = sgn(x)\cdot\log(|x|+1)$ is not used more often as it is like a sigmoid, but doesn't saturate as fast for large $|x|$.

\subsubsection{Step-function}
For the step-function $\sigma(w) =I[aw\geq 0]$ with $a\geq 0$:
\begin{align*}
w = 
\begin{cases}
0 &\mbox{ if }0\leq  \tilde{w} \leq \sqrt{2a\eta}\\
\tilde{w} & \mbox{ otherwise}
\end{cases}
\end{align*}
whereas for vanilla SGD it is $w = \tilde{w}$ always since the gradient is zero. The problem is that gradients cannot back-propagate as they are always zero. This could be dealt with by guaranteeing that from every step-function node there is a path of continuous function nodes (that the errors can back-propagate through). For example each layer could have 10 binary nodes and 1 continuous node, with nodes fully connected between layers. The advantage of the binary nodes is that they should be very fast computationally to execute. Its also possible to have step functions in the very first layer and continuous functions subsequently.

Alternatively one could have shallow networks of just step-functions.

One could ``harden'' a network of ``soft'' activations (like the arctan) by first training with arctan. Then replace each layer of arctans with a layer of step-functions. This could be done by naively replacing or by replacing and then training with the step-function. This must be done bottom up, so the subsequent layers are continuous and can carry the errors. The advantage is that it will be much faster to have a binary network when implementing.

Maybe can define a derivative as the non-Riemannian limit with step size $\eta$? Discrete gradients? This could make the neural network deep. What happens if make the step size random? Then there is a probable gradient with an expectation.

We can also generalize to $k$ steps $\sigma(w) = \sum_{k=1}^KI[w\geq k]$.

Applications:
\begin{itemize}
\item A shallow binary auto-encoder $x\approx f_\theta (x) = C\sigma(Ax+b)+d$.
\item Weighted experts for binary decisions $f_\theta (x) = w^\top \sigma(Ax+b)$ for $w\in\Delta^{K-1}$ where there are $K$ experts (like the Winnow algorithm)
\end{itemize}



The first trick to making the updates fast is to make them one-dimensional. This is achieved by updating just one node at a time:
\begin{align*}
\min_{w}\{2\eta \sigma(a^\top w) + \|w-\tilde{w}\|_2^2\} & = \min_{\epsilon}\{2\eta \sigma(a^\top \tilde{w} + \epsilon\|a\|_2^2) + \epsilon^2\}
\end{align*}
where $w = \tilde{w} +\epsilon \cdot a/\|a\|_2$. 

The next trick is to choose activation functions that can be easily solved for. Such functions include RELU, arctan, ELU and softpus. As shown below, RELU can be solved in closed form, arctan reduces to a cubic equation and ELU and softplus to the Lambert-W. If cannot solve for $\epsilon$ in closed and the gradient of the activation function is bounded by $B$, then the bisection method can be used:
\begin{align*}
- \eta B \leq \epsilon \leq \eta B
\end{align*}
as the bounds would be the greatest possible steps if the gradient was $B$ or $-B$ for all $\theta$. As most activation functions are monotonic, we should be able to set either the upper or lower bound to be zero.

We should probably focus on implementing RELU, arctan, 3-piece-linear-sigmoid, RNN and CNN as these are the most important methods that we can implement.




\subsection{What are the key components of my approach? Also include any specific limitations (and when proposing the idea, any potential difficulties).}
The key idea is to use Implicit Stochastic Gradient Descent (ISGD) for neural networks. ISGD cannot be naively applied, since optimizing the resultant implicit equations would be hard. To make the optimization easier, we make two simplifications:
\begin{enumerate}
\item The ISGD updates are done separately for each parameter. Let $\theta\in\mathbb{R}^p$ be the parameter space. When updating parameter $\theta_k$ the parameters $\theta_{-k}\in\mathbb{R}^{p-1}$ are kept fixed.

The advantage of this scheme is that it makes optimization more tractable. The disadvantage is that it is we only use information along the coordinate axes.

\item The ISGD updates use a combination of linear and non-linear approximations to the deep neural network. Let the neural network with $d$ layers be represented as 
\begin{align*}
f_\theta(x) =&~ g_{\theta_d}^{(d)}(g_{\theta_{d-1}}^{(d-1)}(... g_{\theta_1}^{(1)}(x)...)) \\
=&~ g_{\theta_d}^{(d)}(z_d) \\
&~ s.t.~\,z_d = g_{\theta_{d-1}}^{(d-1)}(z_{d-1})\\
&\qquad z_{d-1} = g_{\theta_{d-2}}^{(d-2)}(z_{d-2})\\
&\qquad ...\\
&\qquad z_{2} = g_{\theta_{1}}^{(1)}(z_{1})\\
&\qquad z_{1} = x
\end{align*}

Let $\tilde{\theta}$ and $\tilde{z}$ denote the current values of $\theta$ and $z$. For $\theta\approx \tilde{\theta}$ we can approximate $f_\theta(x)$ using linear approximations of $z_k$:
\begin{align*}
z_{k+1} &= g_{\theta_{k}}^{(k)}(z_{k})\\
&\approx \tilde{z}_{k+1} + \frac{\partial g_{\tilde{\theta}_{k}}^{(k)}}{\partial z_{k}}\bigg|_{z_{k} = \tilde{z}_{k}}(z_k - \tilde{z}_{k})
\end{align*}
In the future we will drop the conditioning $|_{z_{k} = \tilde{z}_{k}}$ when it is clear from the context.
We could apply these linear approximations to any given $z_k$ set of $z_k$'s. The more $z_k$ we apply it to, the worse the approximation becomes. 

Now let us consider updating parameter $\theta_k$. Layers $1,...,k$ are not affected by a change in $\theta_k$ and so we can fix them to their current values. Layers $k+1,...,d$ do depend on $\theta_k$. In our proposed method we will simplify this dependence by linearizing layers $k+2,...,d$. Denoting this approximation as $h_{\theta_k,\tilde{z}}^{(k)}(x) \approx f_{\theta_k,\tilde{\theta}_{-k}}(x)$,
\begin{align*}
h_{\theta_k,\tilde{z}}^{(k)}(x)=&~ f_{\tilde{\theta}}(x) + \frac{\partial g_{\tilde{\theta}_{d}}^{(d)}}{\partial z_{d}}(z_d - \tilde{z}_d) \\
&~ s.t.~\,z_d = \tilde{z}_{d} + \frac{\partial g_{\tilde{\theta}_{d-1}}^{(d-1)}}{\partial z_{d-1}}(z_{d-1} - \tilde{z}_{d-1})\\
&\qquad ...\\
&\qquad z_{k+2} = \tilde{z}_{k+1} + \frac{\partial g_{\tilde{\theta}_{k+1}}^{(k+1)}}{\partial z_{k+1}}(z_{k+1} - \tilde{z}_{k+1})\\
&\qquad z_{k+1} = g_{\theta_{k}}^{(k)}(\tilde{z}_{k})\\
=&~ f_{\tilde{\theta}}(x) + \frac{\partial g_{\tilde{\theta}_{d}}^{(d)}}{\partial z_{d}}\frac{\partial g_{\tilde{\theta}_{d-1}}^{(d-1)}}{\partial z_{d-1}}...\frac{\partial g_{\tilde{\theta}_{k+1}}^{(k+1)}}{\partial z_{k+1}}(g_{\theta_{k}}^{(k)}(\tilde{z}_{k})- \tilde{z}_{k+1}).
\end{align*}
It has derivative:
\begin{equation*}
\nabla_{\theta_k} h_{\theta_k,\tilde{z}}^{(k)}(x) = \frac{\partial g_{\tilde{\theta}_{d}}^{(d)}}{\partial z_{d}}\frac{\partial g_{\tilde{\theta}_{d-1}}^{(d-1)}}{\partial z_{d-1}}...\frac{\partial g_{\tilde{\theta}_{k+1}}^{(k+1)}}{\partial z_{k+1}}\nabla_{\theta_k} g_{\theta_{k}}^{(k)}(\tilde{z}_{k}).
\end{equation*}
As a sanity check note that the value and first derivative of $h_{\theta_k,\tilde{z}}^{(k)}(x)$ matches that of $f_{\theta_k,\tilde{\theta}_{-k}}(x)$ at $\theta_k = \tilde{\theta}_k$.

Instead of doing ISGD on $f_{\theta_k,\tilde{\theta}_{-k}}(x)$ we will do it on $h_{\theta_k,\tilde{z}}^{(k)}(x)$. Note that if we had also linearized layer $k+1$, then ISGD on $h$ would be equivalent to vanilla SGD. We could also have chosen to not linearize another layer $j>k+1$ and instead linearize layer $k+1$, in which case the approximation would be
\begin{align*}
h_{\theta_k,\tilde{z}}^{(k,j)}(x)=& f_{\tilde{\theta}}(x) + \frac{\partial g_{\tilde{\theta}_{d}}^{(d)}}{\partial z_{d}}...\frac{\partial g_{\tilde{\theta}_{j+1}}^{(j+1)}}{\partial z_{j+1}}\\
&\cdot \left(g_{\theta_{j}}^{(j)}(\tilde{z}_{j} + \frac{\partial g_{\tilde{\theta}_{j-1}}^{(j-1)}}{\partial z_{j-1}}...\frac{\partial g_{\tilde{\theta}_{k+1}}^{(k+1)}}{\partial z_{k+1}} \nabla_{\theta_k} g_{\theta_k}^{(k)}(\tilde{z}_k)\bigg|_{\theta_k = \tilde{\theta}_k}(\theta_{k} - \tilde{\theta}_{k}))- \tilde{z}_{j+1}\right).
\end{align*}
Ideally we should choose the $j\geq k+1$ that has the greatest curvature (but selecting such a $j$ is a conditioning procedure that might break the convergence properties).
